Effective pruning of web-scale datasets based on complexity of concept clusters

Utilizing massive web-scale datasets has led to unprecedented performance gains in machine learning models, but also imposes outlandish compute requirements for their training. In order to improve training and data efficiency, we here push the limits of pruning large-scale multimodal datasets for training CLIP-style models. Today's most effective pruning method on ImageNet clusters data samples into separate concepts according to their embedding and prunes away the most prototypical samples. We scale this approach to LAION and improve it by noting that the pruning rate should be concept-specific and adapted to the complexity of the concept. Using a simple and intuitive complexity measure, we are able to reduce the training cost to a quarter of regular training. By filtering from the LAION dataset, we find that training on a smaller set of high-quality data can lead to higher performance with significantly lower training costs. More specifically, we are able to outperform the LAION-trained OpenCLIP-ViT-B32 model on ImageNet zero-shot accuracy by 1.1p.p. while only using 27.7% of the data and training compute. Despite a strong reduction in training cost, we also see improvements on ImageNet dist. shifts, retrieval tasks and VTAB. On the DataComp Medium benchmark, we achieve a new state-of-the-art Imagehttps://info.arxiv.org/help/prep#commentsNet zero-shot accuracy and a competitive average zero-shot accuracy on 38 evaluation tasks.

==> Tables/class-balance-ratio.tex <==
\begin{table*}[tb]
\small
\centering
\caption{The class-balance ratio is an important hyperparameter of SSP-Pruning.}
 \label{tab:cls_bal}

\begin{tabular}{l c c }
\toprule
Class-balance ratio & Top1 accuracy [\%] &  Top5 accuracy\\
0.5 & \\
0.9 & \\
\bottomrule
\end{tabular}

\end{table*}

==> Tables/datacomp_results.tex <==
\definecolor{LightCyan}{rgb}{0.75,1,1}
\definecolor{LightGray}{rgb}{0.95,0.95,0.95}
\definecolor{LightGreen}{rgb}{0.67, 0.88, 0.69}
% \newcolumntype{g}[1]{>{\columncolor{LightGray}}c|}



\begingroup

\setlength{\tabcolsep}{4.5pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.3} % Default value: 1
\begin{table*}[tb]

\small
\centering
\caption{Our approach outperforms the current state of the art on DataComp Medium (T-MARS) on most tasks.}
 \label{tab:datacom_result}

% \begin{tabular}{llrrrrr}
%\resizebox{1.\textwidth}{!}{

\begin{tabular}{l r|cc|ccc}  %{C{3.cm}|C{2.cm}|C{2.cm}C{1.cm}C{2.cm}C{2.cm}|C{2.cm}}

\toprule
Method & Size &  ImageNet &  ImageNet dist. shifts &   VTAB &  Retrieval &  Average \\
\midrule
TMARS \citep{maini2023t}                                              &  25M &     33.00 &                  \colorbox{LightGreen}{27.00} &  36.30 &      22.50 &    \colorbox{LightGreen}{36.10} \\

% Ours &  0.0 &     31.56 &                  25.14 &  37.55 &      26.68 &    35.06 \\


Image-based $\cap$ CLIP Score (L/14 top 30\%)  \citet{gadre2023datacomp}                        &  14M &     29.70 &                  23.90 &  34.60 &      23.10 &    32.80 \\
CLIP Score (L/14 top 30\%)  \citet{gadre2023datacomp}                                    &  38M &     27.30 &                  23.00 &  33.80 &      25.10 &    32.80 \\

Ours (DeDup, 80\% + CLIP-L/14 Score, 50\% + CBP) &  19.2M &     \colorbox{LightGreen}{33.35} &                  24.73 &  \colorbox{LightGreen}{37.26} &      \colorbox{LightGreen}{26.82} &    34.52 \\
Ours (DeDup, 80\% + CLIP-L/14 Score, 40\% + CBP) &  19M &     32.02 &                 25.74 &  \colorbox{LightGreen}{37.26} &      26.80 &    35.33 \\

\bottomrule
\end{tabular}
%}

\end{table*}

\endgroup


==> Tables/datacomp_results_iclr.tex <==
\definecolor{LightCyan}{rgb}{0.75,1,1}
\definecolor{LightGray}{rgb}{0.95,0.95,0.95}
\definecolor{LightGreen}{rgb}{0.67, 0.88, 0.69}
% \newcolumntype{g}[1]{>{\columncolor{LightGray}}c|}



\begingroup

\setlength{\tabcolsep}{1pt} % Default value: 6pt
%\renewcommand{\arraystretch}{1.3} % Default value: 1
\begin{table*}[tb]

\small
\centering
\caption{Our approach outperforms the current state of the art on DataComp Medium (T-MARS) on most tasks.}
 \label{tab:datacom_result}

% \begin{tabular}{llrrrrr}
%\resizebox{1.\textwidth}{!}{

\begin{tabular}{l r|cc|ccc}  %{C{3.cm}|C{2.cm}|C{2.cm}C{1.cm}C{2.cm}C{2.cm}|C{2.cm}}

\toprule
Method & Size &  ImageNet &  ImageNet dist. shifts &   VTAB &  Retrieval &  Average \\
\midrule
TMARS                                              &  25M &     33.00 &                  \colorbox{LightGreen}{27.00} &  36.30 &      22.50 &    \colorbox{LightGreen}{36.10} \\

% Ours &  0.0 &     31.56 &                  25.14 &  37.55 &      26.68 &    35.06 \\


Image-based $\cap$ CLIP Score (L/14 top 30\%)                        &  14M &     29.70 &                  23.90 &  34.60 &      23.10 &    32.80 \\
CLIP Score (L/14 top 30\%)                                     &  38M &     27.30 &                  23.00 &  33.80 &      25.10 &    32.80 \\

Ours (DeDup, 80\% + CLIP-L/14 Score, 50\% + CBP) &  19.2M &     \colorbox{LightGreen}{33.35} &                  24.73 &  \colorbox{LightGreen}{37.26} &      \colorbox{LightGreen}{26.82} &    34.52 \\
Ours (DeDup, 80\% + CLIP-L/14 Score, 40\% + CBP) &  19M &     32.02 &                 25.74 &  \colorbox{LightGreen}{37.26} &      26.80 &    35.33 \\

\bottomrule
\end{tabular}
%}

\end{table*}

\endgroup


==> Tables/deduplication_plus_clip_score_table.tex <==
\begin{table}[tb]
\small
\setlength{\tabcolsep}{2pt}

\centering
\caption{CLIP score filtering is more effective after deduplication on DataComp Medium.}
 \label{tab:deduplication_plus_clip_score}

\begin{tabular}{lc|ccc}
\toprule


DeDup. & Pool Size & Dataset Size & IN top1 acc. &  average acc.  \\
\midrule
No           & 128M & 38M &  27.30    & 32.80  \\
Yes, to 80\% & 120M & 38M & \colorbox{LightGreen}{27.93}     & \colorbox{LightGreen}{33.03} \\

\bottomrule
\end{tabular}



\end{table}

==> Tables/final_hparams_together.tex <==
\begin{table*}[tb]
\centering
\caption{The number of clusters is an important hyperparameter of SSP-Pruning.}
 \label{tab:number_of_clusters}

\begin{tabular}{l c c }
\toprule
Number of clusters & Top1 accuracy [\%] &  Top5 accuracy\\
1k & \\
10k & \\
\bottomrule
\end{tabular}

\centering
\caption{The class-balance ratio is an important hyperparameter of SSP-Pruning.}
 \label{tab:cls_bal}

\begin{tabular}{l c c }
\toprule
Class-balance ratio & Top1 accuracy [\%] &  Top5 accuracy\\
0.5 & \\
0.9 & \\
\bottomrule
\end{tabular}

\centering
\caption{The temperature is an important hyperparameter of CB-pruning.}
 \label{tab:temperature}

\begin{tabular}{l c c }
\toprule
Temperature & Top1 accuracy [\%] &  Top5 accuracy\\
0.1 & \\
0.5 & \\
0.9 & \\
\bottomrule
\end{tabular}

\end{table*}

==> Tables/image_encoder.tex <==
\begin{table*}[tb]
%\small
\centering
\caption{The choice of the image encoder influences the performance of SSP-Pruning.}
 \label{tab:image_encoder}

\begin{tabular}{l c c }
\toprule
Image encoder & Top1 accuracy [\%] &  Top5 accuracy\\
ViT-XY DinoV2 \citep{oquab2023dinov2} & \\
ViT-XY CLIP & \\
\bottomrule
\end{tabular}

\centering
\caption{The choice of the text encoder influences the performance of SSP-Pruning.}
 \label{tab:text_encoder}

\begin{tabular}{l c c }
\toprule
Text encoder & Top1 accuracy [\%] &  Top5 accuracy\\
ViT-XY BERT \citep{devlin-etal-2019-bert} & \\
ViT-XY CLIP & \\
\bottomrule
\end{tabular}

\end{table*}

==> Tables/laion50m_results_table.tex <==
\definecolor{LightCyan}{rgb}{0.75,1,1}
\definecolor{LightGray}{rgb}{0.95,0.95,0.95}
\definecolor{LightGreen}{rgb}{0.67, 0.88, 0.69}
% \newcolumntype{g}[1]{>{\columncolor{LightGray}}c|}



\begingroup

\setlength{\tabcolsep}{4.5pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.3} % Default value: 1
\begin{table*}[tb]

\small
\centering
\caption{Result on LAION50M dataset}
 \label{tab:datacom_result}

% \begin{tabular}{llrrrrr}
\resizebox{1.\textwidth}{!}{

\begin{tabular}{C{3.cm}|C{2.cm}|C{2.cm}C{1.cm}C{2.cm}C{2.cm}|C{2.cm}}

\toprule
Method & Size &  ImageNet &  ImageNet dist. shifts &   VTAB &  Retrieval &  Average \\
\midrule
TMARS \citet{maini2023t}                                              &  25M &     33.00 &                  27.00 &  36.30 &      22.50 &    \colorbox{LightGreen}{36.10} \\

Ours (DeDup, 80\% - CLIP Score, 50\% - DBP) &  19.2M &     \colorbox{LightGreen}{33.35} &                  24.73 &  37.26 &      26.82 &    34.52 \\
Ours (DeDup, 80\% - CLIP Score, 40\% - DBP) &  19M &     32.02 &                  25.74 &  37.26 &      26.80 &    35.33 \\
% Ours &  0.0 &     31.56 &                  25.14 &  37.55 &      26.68 &    35.06 \\


Image-based $\cap$ CLIP Score (L/14 top 30\%) \citet{gadre2023datacomp}                        &  14M &     29.70 &                  23.90 &  34.60 &      23.10 &    32.80 \\
CLIP Score (L/14 top 30\%) \citet{gadre2023datacomp}                                    &  38M &     27.30 &                  23.00 &  33.80 &      25.10 &    32.80 \\
\bottomrule
\end{tabular}
}

\end{table*}

\endgroup


==> Tables/modality.tex <==
\begin{table*}[tb]
\small
\centering
\caption{The modality of the embeddings influences the performance of SSP-Pruning.}
 \label{tab:modality}

\begin{tabular}{l c c }
\toprule
Embeddings modality & Top1 accuracy [\%] &  Top5 accuracy\\
Image only & \\
Text only & \\
Multi-modal (BLIP \citep{li2022blip}) & \\
Aggregated & \\
\bottomrule
\end{tabular}

\end{table*}

==> Tables/model_size_table.tex <==
\definecolor{LightCyan}{rgb}{0.75,1,1}
\definecolor{LightGray}{rgb}{0.95,0.95,0.95}
\definecolor{LightGreen}{rgb}{0.67, 0.88, 0.69}
% \newcolumntype{g}[1]{>{\columncolor{LightGray}}c|}


\begin{table}[tb]
\small
\setlength{\tabcolsep}{4pt}
\centering
\caption{CBP outperforms CLIP score filtering across different model sizes on LAION-50M. All models are trained for 5 epochs.}
 \label{tab:model_size_results}

\resizebox{0.48\textwidth}{!}{%

\begin{tabular}{l|cccc}
\toprule

 & Dataset & CLIP-S/32 & CLIP-B/32 & CLIP-L/14  \\
Method/Model. &  Size & IN top1 acc & IN top1 acc & IN top1 acc  \\
\midrule

CLIP score & 30M    & 32.32 &  38.07    & 47.61  \\
CB-Pruning & 30M & \colorbox{LightGreen}{39.04} &  \colorbox{LightGreen}{43.41}     &  \colorbox{LightGreen}{53.21} \\

\bottomrule
\end{tabular}
}

\vspace{-3mm}

\end{table}

==> Tables/number_of_clusters.tex <==
\begin{table*}[tb]
\small
\centering
\caption{The number of clusters is an important hyperparameter of SSP-Pruning.}
 \label{tab:number_of_clusters}

\begin{tabular}{l c c }
\toprule
Number of clusters & Top1 accuracy [\%] &  Top5 accuracy\\
1k & \\
10k & \\
\bottomrule
\end{tabular}

\end{table*}

==> Tables/ssp_pruning_vs_cbp.tex <==
\begin{table}[tb]
\setlength{\tabcolsep}{4pt}
\small
\centering
\caption{Complexity-based pruning (CBP) helps improve the performance of SSP-Pruning. We prune the LAION-50M dataset to 30M examples and train CLIP-B/32 on it for 5 epochs. We use 500 clusters and set the cluster balancing value of SSP-Pruning method to 1.0.
% D data is a necessary precursor to performing SSP-Pruning on DataComp Medium.
}
 \label{tab:ssp_pruning_vs_cbp}

\begin{tabular}{l|ccc}
\toprule

Method/ # K-means clusters &  10,000 clusters & 500 clusters \\
\midrule

CBP           & \colorbox{LightGreen}{41.61} & \colorbox{LightGreen}{43.41} \\  
SSP-Pruning &          39.01  & 42.91    \\
\bottomrule
\end{tabular}



\end{table}

==> Tables/temperature.tex <==
\begin{table*}[tb]
\small
\centering
\caption{The temperature is an important hyperparameter of CB-pruning.}
 \label{tab:temperature}

\begin{tabular}{l c c }
\toprule
Temperature & Top1 accuracy [\%] &  Top5 accuracy\\
0.1 & \\
0.5 & \\
0.9 & \\
\bottomrule
\end{tabular}

\end{table*}

==> Tables/text_encoder.tex <==
\begin{table*}[tb]
\small
\centering
\caption{The choice of the text encoder influences the performance of SSP-Pruning.}
 \label{tab:text_encoder}

\begin{tabular}{l c c }
\toprule
Text encoder & Top1 accuracy [\%] &  Top5 accuracy\\
ViT-XY BERT \citep{devlin-etal-2019-bert} & \\
ViT-XY CLIP & \\
\bottomrule
\end{tabular}

\end{table*}

==> Tables_ICLR/class-balance-ratio.tex <==
\begin{table*}[tb]
\small
\centering
\caption{The class-balance ratio is an important hyperparameter of SSP-Pruning.}
 \label{tab:cls_bal}

\begin{tabular}{l c c }
\toprule
Class-balance ratio & Top1 accuracy [\%] &  Top5 accuracy\\
0.5 & \\
0.9 & \\
\bottomrule
\end{tabular}

\end{table*}

==> Tables_ICLR/datacomp_results.tex <==
\definecolor{LightCyan}{rgb}{0.75,1,1}
\definecolor{LightGray}{rgb}{0.95,0.95,0.95}
\definecolor{LightGreen}{rgb}{0.67, 0.88, 0.69}
% \newcolumntype{g}[1]{>{\columncolor{LightGray}}c|}



\begingroup

\setlength{\tabcolsep}{4.5pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.3} % Default value: 1
\begin{table*}[tb]

\small
\centering
\caption{Our approach outperforms the current state of the art on DataComp Medium (T-MARS) on most tasks.}
 \label{tab:datacom_result}

% \begin{tabular}{llrrrrr}
%\resizebox{1.\textwidth}{!}{

\begin{tabular}{l r|cc|ccc}  %{C{3.cm}|C{2.cm}|C{2.cm}C{1.cm}C{2.cm}C{2.cm}|C{2.cm}}

\toprule
Method & Size &  ImageNet &  ImageNet dist. shifts &   VTAB &  Retrieval &  Average \\
\midrule
TMARS \citep{maini2023t}                                              &  25M &     33.00 &                  \colorbox{LightGreen}{27.00} &  36.30 &      22.50 &    \colorbox{LightGreen}{36.10} \\

% Ours &  0.0 &     31.56 &                  25.14 &  37.55 &      26.68 &    35.06 \\


Image-based $\cap$ CLIP Score (L/14 top 30\%)  \citet{gadre2023datacomp}                        &  14M &     29.70 &                  23.90 &  34.60 &      23.10 &    32.80 \\
CLIP Score (L/14 top 30\%)  \citet{gadre2023datacomp}                                    &  38M &     27.30 &                  23.00 &  33.80 &      25.10 &    32.80 \\

Ours (DeDup, 80\% + CLIP-L/14 Score, 50\% + CBP) &  19.2M &     \colorbox{LightGreen}{33.35} &                  24.73 &  \colorbox{LightGreen}{37.26} &      \colorbox{LightGreen}{26.82} &    34.52 \\
Ours (DeDup, 80\% + CLIP-L/14 Score, 40\% + CBP) &  19M &     32.02 &                 25.74 &  \colorbox{LightGreen}{37.26} &      26.80 &    35.33 \\

\bottomrule
\end{tabular}
%}

\end{table*}

\endgroup


==> Tables_ICLR/deduplication_table.tex <==
\begin{table}[tb]
\setlength{\tabcolsep}{4pt}
\small
\centering
\caption{DBP is more effective on deduplicated vs non-deduplicated DataComp Medium. The result holds for two different dataset sizes.
We did not apply CLIP score filtering in this experiment.
% D data is a necessary precursor to performing SSP-Pruning on DataComp Medium.
}
 \label{tab:deduplication}
\resizebox{0.65\textwidth}{!}{%

\begin{tabular}{l|ccc}
\toprule


% Pruning method & Top1 accuracy [\%] &  Top5 accuracy\\
% SSP-Pruning without deduplication & \\
% SSP-Pruning with deduplication & \\
Deduplicated? & DBP, Dataset Size (M) & ImageNet top-1 acc. &  Average acc.  \\
\midrule

No           & 48M &  20.70    & 27.00  \\
Yes, to 80\% & 48M & \colorbox{LightGreen}{21.34}    &  \colorbox{LightGreen}{27.71} \\
\midrule
No           & 24M & 19.10     & 26.10 \\
Yes, to 80\% & 24M & \colorbox{LightGreen}{20.16}    & \colorbox{LightGreen}{27.30}  \\
\bottomrule
\end{tabular}
}


\end{table}

==> Tables_ICLR/final_hparams_together.tex <==
\begin{table*}[tb]
\centering
\caption{The number of clusters is an important hyperparameter of SSP-Pruning.}
 \label{tab:number_of_clusters}

\begin{tabular}{l c c }
\toprule
Number of clusters & Top1 accuracy [\%] &  Top5 accuracy\\
1k & \\
10k & \\
\bottomrule
\end{tabular}

\centering
\caption{The class-balance ratio is an important hyperparameter of SSP-Pruning.}
 \label{tab:cls_bal}

\begin{tabular}{l c c }
\toprule
Class-balance ratio & Top1 accuracy [\%] &  Top5 accuracy\\
0.5 & \\
0.9 & \\
\bottomrule
\end{tabular}

\centering
\caption{The temperature is an important hyperparameter of CB-pruning.}
 \label{tab:temperature}

\begin{tabular}{l c c }
\toprule
Temperature & Top1 accuracy [\%] &  Top5 accuracy\\
0.1 & \\
0.5 & \\
0.9 & \\
\bottomrule
\end{tabular}

\end{table*}

==> Tables_ICLR/image_encoder.tex <==
\begin{table*}[tb]
%\small
\centering
\caption{The choice of the image encoder influences the performance of SSP-Pruning.}
 \label{tab:image_encoder}

\begin{tabular}{l c c }
\toprule
Image encoder & Top1 accuracy [\%] &  Top5 accuracy\\
ViT-XY DinoV2 \citep{oquab2023dinov2} & \\
ViT-XY CLIP & \\
\bottomrule
\end{tabular}

\centering
\caption{The choice of the text encoder influences the performance of SSP-Pruning.}
 \label{tab:text_encoder}

\begin{tabular}{l c c }
\toprule
Text encoder & Top1 accuracy [\%] &  Top5 accuracy\\
ViT-XY BERT \citep{devlin-etal-2019-bert} & \\
ViT-XY CLIP & \\
\bottomrule
\end{tabular}

\end{table*}

==> Tables_ICLR/laion50m_results_table.tex <==
\definecolor{LightCyan}{rgb}{0.75,1,1}
\definecolor{LightGray}{rgb}{0.95,0.95,0.95}
\definecolor{LightGreen}{rgb}{0.67, 0.88, 0.69}
% \newcolumntype{g}[1]{>{\columncolor{LightGray}}c|}



\begingroup

\setlength{\tabcolsep}{4.5pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.3} % Default value: 1
\begin{table*}[tb]

\small
\centering
\caption{Result on LAION50M dataset}
 \label{tab:datacom_result}

% \begin{tabular}{llrrrrr}
\resizebox{1.\textwidth}{!}{

\begin{tabular}{C{3.cm}|C{2.cm}|C{2.cm}C{1.cm}C{2.cm}C{2.cm}|C{2.cm}}

\toprule
Method & Size &  ImageNet &  ImageNet dist. shifts &   VTAB &  Retrieval &  Average \\
\midrule
TMARS \citet{maini2023t}                                              &  25M &     33.00 &                  27.00 &  36.30 &      22.50 &    \colorbox{LightGreen}{36.10} \\

Ours (DeDup, 80\% - CLIP Score, 50\% - DBP) &  19.2M &     \colorbox{LightGreen}{33.35} &                  24.73 &  37.26 &      26.82 &    34.52 \\
Ours (DeDup, 80\% - CLIP Score, 40\% - DBP) &  19M &     32.02 &                  25.74 &  37.26 &      26.80 &    35.33 \\
% Ours &  0.0 &     31.56 &                  25.14 &  37.55 &      26.68 &    35.06 \\


Image-based $\cap$ CLIP Score (L/14 top 30\%) \citet{gadre2023datacomp}                        &  14M &     29.70 &                  23.90 &  34.60 &      23.10 &    32.80 \\
CLIP Score (L/14 top 30\%) \citet{gadre2023datacomp}                                    &  38M &     27.30 &                  23.00 &  33.80 &      25.10 &    32.80 \\
\bottomrule
\end{tabular}
}

\end{table*}

\endgroup


==> Tables_ICLR/markdown_table9.tex <==
|  |  | Image-based & CLIP-score | DeDup,80% | DeDup,80% |
|---|---|---|---|---|
|  |  | (L/14 top 30%) | +CLIP Score,40% | +CLIP-score,50% |
| Dataset | Metric | | +DBP | +DBP |
| Caltech-101 | top-1 acc | 71.59 | **74.35** | 74.02 |
| CIFAR-10 | top-1 acc | 82.52 | 84.66 | **85.91** |
| CIFAR-100  | top-1 acc | 54.76 | 58.54 | **59.34** |
| CLEVR Counts | top-1 acc | 13.65 | 14.58 | **16.38** |
| CLEVR Distance | top-1 acc | 22.49 | 22.37 | **23.62** |
| Country211 | top-1 acc | 4.53 | 5.55 | **6.0** |
| Describable Textures | top-1 acc | 21.33 | 22.18 | **23.35** |
| EuroSAT | top-1 acc | 33.93 | **35.98** | 34.22 |
| FGVC Aircraft | top-1 acc | 3.04 | 3.39 | **3.87** |
| Food-101   | top-1 acc | 41.68 | 46.99 | **49.07** |
| GTSRB | top-1 acc | **13.66** | 11.77 | 10.17 |
| ImageNet 1k | top-1 acc | 29.72 | 32.02 | **33.35** |
| ImageNet Sketch  | top-1 acc | 19.3 | **20.17** | 17.73 |
| ImageNet v2 | top-1 acc | 24.4 | 26.54 | **28.34** |
| ImageNet-A  | top-1 acc | 4.93 | 5.57 | **6.45** |
| ImageNet-O   | top-1 acc | 40.85 | **43.75** | 42.7 |
| ImageNet-R      | top-1 acc | 34.02 | **35.46** | 32.78 |
| KITTI Vehicle Distance | top-1 acc | 21.1 | 30.8 | **36.57** |
| MNIST  | top-1 acc | 11.47 | **14.77** | 10.06 |
| ObjectNet | top-1 acc | 19.71 | **22.95** | 20.36 |
| Oxford Flowers-102  | top-1 acc | 29.65 | 34.36 | **36.33** |
| Oxford-IIIT Pet| top-1 acc | 43.11 | 45.82 | **47.4** |
| Pascal VOC 2007 | top-1 acc | 54.59 | 67.47 | **71.83** |
| PatchCamelyon | top-1 acc | 58.62 | **59.58** | 48.9 |
| Rendered SST2  | top-1 acc | **53.16** | 50.58 | 50.14 |
| RESISC45    | top-1 acc | 27.78 | 29.83 | **30.92** |
| Stanford Cars   | top-1 acc | 28.03 | **31.14** | 28.53 |
| STL-10  | top-1 acc | 83.65 | 84.21 | **86.21** |
| SUN397  | top-1 acc | 36.37 | 43.35 | **45.08** |
| SVHN  | top-1 acc | 15 | **16.97** | 14.01 |
| Flickr  | mean recall @1 | 18.12 | **27.46** | 26.85 |
| MSCOCO   |mean recall @1 | 11.0 | **16.78** | 16.45 |
| WinoGAViL| avg. Jaccard score | 43.37 | 45.76 | **46.27** |
| iWildCam | top-1 acc | 1.42 | **13.49** | 7.84 |
| Camelyon17  | top-1 acc | 66.69 | **73.5** | 47.72 |
| FMoW    | top-1 acc | 0.0 | **8.19** | 7.54 |
| Dollar Street  | top-1 acc | **44.98** | 38.11 | 37.97 |
| GeoDE  | top-1 acc | 65.59 | **72.48** | 69.34 |
| Average |  | 32.89 | **35.35** | 34.52 |


==> Tables_ICLR/modality.tex <==
\begin{table*}[tb]
\small
\centering
\caption{The modality of the embeddings influences the performance of SSP-Pruning.}
 \label{tab:modality}

\begin{tabular}{l c c }
\toprule
Embeddings modality & Top1 accuracy [\%] &  Top5 accuracy\\
Image only & \\
Text only & \\
Multi-modal (BLIP \citep{li2022blip}) & \\
Aggregated & \\
\bottomrule
\end{tabular}

\end{table*}

==> Tables_ICLR/model_size_table.tex <==
\definecolor{LightCyan}{rgb}{0.75,1,1}
\definecolor{LightGray}{rgb}{0.95,0.95,0.95}
\definecolor{LightGreen}{rgb}{0.67, 0.88, 0.69}
% \newcolumntype{g}[1]{>{\columncolor{LightGray}}c|}


\begin{table}[tb]
\small
\setlength{\tabcolsep}{4pt}
\centering
\caption{DBP outperforms CLIP score filtering across different model sizes on LAION-50M. All models are trained for 5 epochs.}
 \label{tab:model_size_results}

\resizebox{0.60\textwidth}{!}{%

\begin{tabular}{l|cccc}
\toprule

 & Dataset & CLIP-S/32  & CLIP-B/32  & CLIP-L/14   \\

Method/Model & Size & (63M params.) & (151M params.) & (428M params.)\\
             &      & IN top1 acc & IN top1 acc & IN top1 acc  \\
\midrule

CLIP score & 30M    & 32.32 &  38.07    & 47.61  \\
DB-Pruning & 30M & \colorbox{LightGreen}{39.04} &  \colorbox{LightGreen}{43.41}     &  \colorbox{LightGreen}{53.21} \\

\bottomrule
\end{tabular}
}

\vspace{-3mm}

\end{table}

==> Tables_ICLR/number_of_clusters.tex <==
\begin{table*}[tb]
\small
\centering
\caption{The number of clusters is an important hyperparameter of SSP-Pruning.}
 \label{tab:number_of_clusters}

\begin{tabular}{l c c }
\toprule
Number of clusters & Top1 accuracy [\%] &  Top5 accuracy\\
1k & \\
10k & \\
\bottomrule
\end{tabular}

\end{table*}

==> Tables_ICLR/ssp_pruning_vs_cbp.tex <==
\begin{table}[tb]
\setlength{\tabcolsep}{4pt}
\small
\centering
\caption{Complexity-based pruning (CBP) helps improve the performance of SSP-Pruning. We prune the LAION-50M dataset to 30M examples and train CLIP-B/32 on it for 5 epochs. We set the cluster balancing value of SSP-Pruning method to 1.0.
% D data is a necessary precursor to performing SSP-Pruning on DataComp Medium.
}
 \label{tab:ssp_pruning_vs_cbp}

\begin{tabular}{l|ccc}
\toprule

Method/ # K-means clusters &  10,000 clusters & 500 clusters \\
\midrule

CBP           & \colorbox{LightGreen}{41.61} & \colorbox{LightGreen}{43.41} \\  
SSP-Pruning &          39.01  & 42.91    \\
\bottomrule
\end{tabular}



\end{table}

==> Tables_ICLR/temperature.tex <==
\begin{table*}[tb]
\small
\centering
\caption{The temperature is an important hyperparameter of CB-pruning.}
 \label{tab:temperature}

\begin{tabular}{l c c }
\toprule
Temperature & Top1 accuracy [\%] &  Top5 accuracy\\
0.1 & \\
0.5 & \\
0.9 & \\
\bottomrule
\end{tabular}

\end{table*}

==> Tables_ICLR/text_encoder.tex <==
\begin{table*}[tb]
\small
\centering
\caption{The choice of the text encoder influences the performance of SSP-Pruning.}
 \label{tab:text_encoder}

\begin{tabular}{l c c }
\toprule
Text encoder & Top1 accuracy [\%] &  Top5 accuracy\\
ViT-XY BERT \citep{devlin-etal-2019-bert} & \\
ViT-XY CLIP & \\
\bottomrule
\end{tabular}

\end{table*}
